Measuring and controlling radio-frequency quanta with superconducting circuits

In this PhD thesis, we will present the theoretical and experimental work that led to the realization of a radio-frequency circuit quantum electrodynamics system (RFcQED). In chapter 2, we provide a detailed derivation of the Hamiltonian of circuit QED formulated in the context of the Rabi model, and extract expressions for the cross-Kerr interaction. The resulting requirements for the coupling rate in RFcQED are discussed, one of them being the need to dramatically increase the coupling rate compared to typical circuit QED device. In chapter 3 we cover two experimental approaches to increasing the coupling in a circuit QED system, one making use of a high impedance resonator, the second utilizing a large coupling capacitor. In chapter 4, we combine these two approaches to implement RFcQED. Through strong dispersive coupling, we could measure individual photons in a megahertz resonator, demonstrate quantum control by cooling the resonator to the ground state or preparing Fock states, and finally observe with nanosecond resolution the re-thermalization of these states. In chapter 5 we present QuCAT or Quantum Circuit Analyzer Tool in Python, a software package that can be used for the design of circuit QED systems such as the one presented in this thesis. In chapter 6 we discuss how certain interplays between general relativity and quantum mechanics cannot be described using our current laws of physics. In particular, we show how radio-frequency mechanical oscillators are perfect candidates to perform experiments in this regime. In chapter 7 we present the prospects for coupling such mechanical oscillator to weakly anharmonic superconducting circuits such as the transmon qubit or RFcQED systems.

==> acks/acks.tex <==
% !TEX root = ../dissertation.tex

\chapter*{Acknowledgements}
\markboth{Acknowledgements}{}
\addcontentsline{toc}{chapter}{Acknowledgements}
\label{acknowledgements}

This part of my thesis seems to be the hardest one to write. 
%
How is it possible to duly thank and acknowledge everyone who participated in my success in only a couple of pages?
%


I will start with the people who have mentored me.
%
By giving me advice, supervising my work and providing daily support and encouragement, these people have molded me into the scientist I am today, and have given me the motivation, vision, and the methods which makes this hard work possible.


%
\textbf{Gary}, it is hard to realize that I have spent nearly a fifth of my life working with you.
%
I have many things to thank you for, but one that stands out is the relationship of trust that we have.
%
It has made these years a truly pleasurable experience of discovery and creativity.
%
I still remember being hugely impressed when sitting in on my first lecture by you all those years ago.
%
A student raised his hand and asked a question. You paused for a second to think. And then answered "I don't know!".
%
How unique, I thought, to find a professor with such humility.
%
This is one of your great qualities that I have tried to emulate: you hate BS and are not afraid to admit you don't understand something.
%
When you finally understand (usually faster than anyone else in the room!), your understanding is intuitive and you explanations crystal clear.
%
This has been another lesson for me, to refuse to accept a complicated explanation, because it seems that everything can be explained with masses and springs!
%
But more than a great scientist, I have to applaud the great manager, and human being, that you are.
%
It is evident that you care deeply about people in the group, not only their technical problems but also their personal problems.
%
When someone is struggling, you don't throw in the towel, or push insensitively, but try to understand.
%
Sometimes you invest huge amounts of time in someone, even though there is clearly no personal gain, but because you care.
%
This is truly admirable.
%


%
\textbf{Sal}, you are the reason I started this research in the first place.
%
You recruited me into this group five years ago, with talks of quantum gravity, making the best qubit ever, and many other grand projects.
%
One of which you have now pushed to incredible heights with Delft Circuits.
%
I remember one of our first walks on the campus where you told me "We're going to get the Nobel prize, it will be you, me, and Gary. Think about it, you'll be the first Master student with a Nobel prize". 
%
I was sold.
%
In the end we don't have the Nobel prize yet (even though along the way you told me I would get it for other projects too!), but it doesn't matter, and looking back on it I learned a valuable lesson:
%
If we aren't aiming for the stars, then why the hell are we doing this.
%
Many people are afraid of saying that they are aiming for the stars, afraid of the inevitable reaction "well who do you think you are?". 
%
You seem to be immune to this.
%
With a mad glint in your eye, you explain how what you are doing is going to change the world, you erase the doubt in your auditor and he then wants to reach the stars with you. 
%
I hope to do this half as good as you do some day.
%

%
\textbf{Daniel}, you have been in the group for as long as myself, and have had a huge role in shaping the way I work.
%
You have been a mentor, a daily supervisor, and a friend.
%
With incredible persistence and hard-work, you read through and corrected every word of every draft of our papers.
%
You did this regardless of your responsibilities in other project, and regardless of my arrogant resistance to change.
%
But thanks to you efforts, you succeeded in changing me, and I am now a better scientist.
%
Your scientific ideas and creativity are behind many of the results I presented in this thesis: we made a great team and have a lot to show for it.
%
Your patience, technical competence, and hard-work go however way beyond your contributions to my work, as I think everyone around you is immensely thankful to have you: you seem to have a good answer to most things, and are always available to listen.
%
You have been key to the success of the lab as a whole over these years and you should be very proud of that.

%
Beyond these mentors and friends, here are the other heroes who have made my life such a pleasure.
%


%
\textbf{Marios}, you have been my main man since you moved into my office.
%
It's good that we part ways now, otherwise we run the risk of merging into a single, ontbijt-drinking, jazz-listening, circuit-quantizing, meta-Mario$\sqrt{s}$.
%
You have the toughest job of us all, with a young child at home, but you have succeeded admirably.
%
I have no doubt you will continue to do so.
%
I would like to thank you for your friendship: having such a good friend, not only to work with everyday, but sitting next you, is something to treasure. 
%
It just makes everyday a little better.
%

%
\textbf{Daan}, what a journey this has been since we met on the first days of our Masters and got together for the dispuut.
%
We've had so many adventures together, and I hope we spend many more evenings together retelling them, as well as having more.
%
I am so impressed with what you have done in Delft Circuits, you can be very proud of what you have done.



%
\textbf{Sarwan}, we have also been together since I arrived in the Netherlands.
%
We have studied together, partied together, when I started my MEP, you were there with me, when I started my PhD, you were there too.
%
To be honest I'm scared I'll get to my next country and you'll be there waiting for me in my living room.
%
Throughout the years, I've thoroughly enjoyed your company, and I always have the most interesting and diverse conversations with you.
%
And always remember sir that a cheese cake doesn't count as one of your 5 cheeses.


\textbf{Ines}, it has been lovely sharing my time here in Delft with you.
%
I will cherish all the parties and good times we had together, as well as your support in times of need.
%
You future is looking bright, and I hope you find success.


\textbf{Adrian}, you came in at the end, but still we have a lot of memories and good times to remember together.
%
Thank for being such a kind and caring person, I look forward to continuing our friendship.


%
\textbf{Chris}, the period working on the low-frequency transmon experiment was awesome because of you and Marios.
%
We learned a huge amount from each other and shared the joy of discovery.
%
I always enjoyed learning from you, and enjoyed your company and your friendship. 
%

\textbf{Mark}, you will undoubtedly be featured in this section in many theses to come. 
%
You have been, together with Daniel, true pillars in our group, providing a support which will be appreciated for a long time to come.
%
I have to thank you for all your help over the years, as well as for the good times we had outside the lab.



\textbf{Felix}, our best memories are undoubtedly our time in Boston and New York.
%
What an adventure that was.
%
We got on so well on that trip and I will cherish those good memories.
%
You really look set for happiness now. 
All the best planting that tree.


\textbf{Yildiz}, I'm eternally grateful to you for introducing me to Cansel.
%
I've always appreciated your positive vibe and enthusiasm.
%
I look forward to many more good times with you.


\textbf{Nikos}, March meeting 2019 will be etched in my mind as an all time high of my PhD, one reason being that our group got on so well.
%
At your defense you got the best song ever heard because you are loved by all and bring joy to those around you, thanks for being such a great guy.


%
\textbf{Martijn}, we always had great talks together, I hope your endeavors are going great and you will emerge as a tech guru.
%

\textbf{Byoung-Moo}, \textbf{Fatemeh}, \textbf{Hadi}, \textbf{Shun}, \textbf{Jasper}, and all the students who've joined along the years, \textbf{Wouter}, \textbf{Kevin}, and others, I would like to thank you all for making Steele Lab a great place to work.


I would like to extend a special thanks to the Master and Bachelor students who accompanied me personally along the way.
%
The learning went both ways, and I would especially like to thank them for their patience as I slowly learn the best way to guide others.
%


Chronologically: \textbf{May An} and \textbf{Thomas}, I hope you Bachelor projects was enjoyable and I could give you some taste of research.
%
I thank you for showing me the way in Comsol simulations.
%

\textbf{Rémy}, notre temps ensemble a été court, mais le travail que tu as fait a été un véritable phare dans l'obscurité quelques mois plus tard, lorsque je travaillais sur la théorie pour le radio-frequency transmon.
%
Je te remercie de tous tes efforts et j'espère que tu trouvera le succès que tu mérites sans aucun doute.
%

\textbf{Jacob}, I thoroughly enjoyed the time we spent working together.
%
As we were working through all our failures, I kept thinking you were going to stop showing up. 
%
But you just kept at it.
%
You are such a likable person, your enthusiasm and determination is admirable, and I have not doubt you will find a bright future with these qualities.
%

\textbf{Rick}, I greatly enjoyed working with you for all those months.
%
I would in particular like to thank you for your impressive work in the clean room. 
%
As with Jacob, you were not given an easy task, but you carried it independently, making use of critical thinking in a way which gives me great hopes for your future.
%


\textbf{Rik}, I would like to thank you for making your way through all my wacky ideas.
%
You did a fantastic job, and I took great pleasure working with you.
%
We are undoubtedly going to write a great paper about your work here in the months to come.

%
\textbf{Benjamin}, we only know each other for a few months, but already I have taken pleasure in all of our discussions.
%
Let's keep pushing and make QuCAT even better together.


Many other people outside of the Steele Lab also deserve my thanks for making this experience unique.
%
\textbf{Rob}, our daily sessions of pipe club have been one of the best parts of my day, I look forward to many more.
%
\textbf{Holger}, thanks for contributing to our awesome time in the US.
%
\textbf{Yaroslav}, your door has always been open to answer my theoretical questions, thank you.
%
\textbf{Adrian} (Parra-Rodriguez), I hope we get to renew our experience of working together sometime, or just meet-up for a beer at the next conference.
%
I would like to thank everyone in the department, in particular \textbf{Alessandro}, \textbf{Sefano}, and all the other DiCarlo lab guys, and \textbf{Igor}, \textbf{Andreas}, \textbf{Mortitz} and the rest of G-lab for your company at the lunch table.
%
My thanks to the \textbf{Kavli Nanolab} and everyone there for giving us the tools to do these experiments.
%
And thanks to the support staff \textbf{Marijke}, \textbf{Maria}, \textbf{Heleen}, \textbf{Erika} and \textbf{Etty} for guiding me through purchase orders and reimbursement claims (and for everything else that goes on behind the scenes and that I am not aware of).



My happiness throughout these years has also been ensured by wonderful friends outside of physics.
%
Les amis de longue date que j'aimerais voir plus souvent, \textbf{Helene}, \textbf{Sam}, \textbf{Alex}, \textbf{Robin}, \textbf{Nathanael}, \textbf{Manu}, et tant d'autres.
%
The people I have here in Delft outside of our department and who have made my life better, \textbf{David}, \textbf{Cher}, my Vlamily: \textbf{Samy}, \textbf{Kim} and \textbf{Ramona}.


Et maintenant, la famille.
%
Les meilleurs pour la fin.
%
\textbf{Matthieu} et \textbf{Enzo}, vous ne soupçonnez pas l'importance que vous avez dans ma vie.
%
Dans les coups durs et les meilleurs moments vous avez toujours été là.
%
Cette soutenance est un pas de plus dans ma vie, et je n'accepterais personne d'autre que vous à mes côtés.


I would like to thank \textbf{my family}, for their eternal support.
%
Having traveled and met a few people so far in life, I know I am truly blessed for the love I have received, and continue to receive.
%
In particular, I would like to thank \textbf{my parents}, to whom my thesis is dedicated, and who have always believed in me.



Je remercie \textbf{ma famille} pour son éternel soutien.
%
Ayant voyagé et rencontré quelques personnes jusqu'à présent dans la vie, je sais que je suis vraiment chanceux pour l'amour que j'ai reçu et que je continue de recevoir.
%
Je remercie en particulier \textbf{mes parents}, à qui ma thèse est dédiée, et qui ont toujours cru en moi.



And finally, \textbf{Cansel}.
%
Writing all of this down is a celebration of what has passed, but also signals the start of something new.
%
I feel blessed that you are by my side and that I will be starting this next part of my life with my favorite person.
%


\textit{Delft, 10.03.2020}

==> epilogue/epilogue.tex <==
\chapter*{Epilogue}
\addcontentsline{toc}{chapter}{Epilogue}
\label{epilogue}

This is an optional epilogue.


==> preface/preface.tex <==
\chapter*{Preface}
\addcontentsline{toc}{chapter}{Preface}
\setheader{Preface}
Story of my life

\begin{flushright}
{\makeatletter\itshape
    \@firstname\ \@lastname \\
    Delft, XXX
\makeatother}
\end{flushright}



==> template/acks/acks.tex <==
\chapter*{Acknowledgements}
\addcontentsline{toc}{chapter}{Acknowledgements}
\label{acknowledgements}

This is an optional chapter containing acknowledgements.


==> template/conclusion/conclusion.tex <==
\FloatBarrier\chapter{Conclusion}
\label{conclusion}

This is a concluding chapter explaining the scientific and technical
implications for society of the research findings in considerable detail.


==> template/cv/cv.tex <==
\chapter*{Curriculum Vit\ae}
\addcontentsline{toc}{chapter}{Curriculum Vit\ae}
\setheader{Curriculum Vit\ae}

%% Print the full name of the author.
\makeatletter
\authors{\@firstname\ {\titleshape\@lastname}}
\makeatother

\noindent
\begin{tabular}{p{4\parindent}l}
    14-03-1879 & Born in Ulm, Germany.
\end{tabular}

\section*{Education}

\begin{tabular}{p{4\parindent}l}
    1892--1896 & Grammar School \\
    & Luitpold Gymnasium, M\"unich (1892--1895)\\
    & Aurau, Switzerland (1895--1896) \\
    \\
    1896--1900 & Undergraduate in Mathematics \& Physics \\
    & Eidgen\"ossische Polytechnische Schule Z\"urich \\
    \\
    1905 & PhD.\ Physics \\
    & Eidgen\"ossische Polytechnische Schule Z\"urich \\
    &
    %% The width of the second column is the width of the page, minus the width
    %% of the first column (4\parindent) minus four times the separation between
    %% the start of the column and its contents.
    \begin{minipage}{\textwidth-4\parindent-4\tabcolsep}
        %% We divide the minipage 20/80.
        \begin{tabular}{@{}p{0.2\linewidth}@{}p{0.8\linewidth-\tabcolsep}}
            \textit{Thesis:} & Eine neue Bestimmung der Molek\"uldimensionen \\
            \textit{Promotor:} & Prof.\ dr.\ A.\ Kleiner
        \end{tabular}
    \end{minipage}
\end{tabular}

\section*{Awards}

\begin{tabular}{p{4\parindent}l}
    1922 & Nobel Prize in Physics \\
    \\
    1925 & Copley Medal \\
    \\
    1929 & Max Planck Medal \\
    \\
    1999 & Time magazine's person of the century
\end{tabular}



==> template/epilogue/epilogue.tex <==
\chapter*{Epilogue}
\addcontentsline{toc}{chapter}{Epilogue}
\label{epilogue}

This is an optional epilogue.


==> template/preface/preface.tex <==
\chapter*{Preface}
\addcontentsline{toc}{chapter}{Preface}
\setheader{Preface}

Preface goes here. This chapter is optional.

\begin{flushright}
{\makeatletter\itshape
    \@firstname\ \@lastname \\
    Delft, January 2013
\makeatother}
\end{flushright}



==> template/publications/publications.tex <==
\chapter*{List of Publications}
\addcontentsline{toc}{chapter}{List of Publications}
\setheader{List of Publications}
\label{publications}

%% We use the 'etaremune' environment (the reverse of 'enumerate') to get a
%% numbered list of publications in reverse chronological order. If the list of
%% authors is long, it might be useful to emphasize your own name with \textbf.
\begin{etaremune}{\small

\item \textbf{A.\ Einstein}, \textit{Ist die Tr\"agheit eines K\"orpers von seinem Energieinhalt abh\"angig?}, \href{http://dx.doi.org/10.1002/andp.19053231314}{Annalen der Physik \textbf{18}, 639 (1906)}.
\item \textbf{A.\ Einstein}, \textit{Zur Elektrodynamik bewegter K\"orper}, \href{http://dx.doi.org/10.1002/andp.19053221004}{Annalen der Physik \textbf{17}, 891 (1905)}.
\item \textbf{A.\ Einstein}, \textit{\"Uber die von der molekularkinetischen Theorie der W\"arme geforderte Bewegung von in ruhenden Fl\"ussigkeiten suspendierten Teilchen}, \href{http://dx.doi.org/10.1002/andp.19053220806}{Annalen der Physik \textbf{17}, 549 (1905)}.
\item \textbf{A.\ Einstein}, \textit{\"Uber einen die Erzeugung und Verwandlung des Lichtes betreffenden heuristischen Gesichtspunkt}, \href{http://dx.doi.org/10.1002/andp.19053220806}{Annalen der Physik \textbf{17}, 132 (1905)}.

}\end{etaremune}



==> template/summary/summary.tex <==
\chapter*{Summary}
\addcontentsline{toc}{chapter}{Summary}
\setheader{Summary}

Summary in English\ldots

\chapter*{Samenvatting}
\addcontentsline{toc}{chapter}{Samenvatting}
\setheader{Samenvatting}

{\selectlanguage{dutch}

Samenvatting in het Nederlands\ldots

}



==> template/title/title.tex <==
\begin{titlepage}

\begin{center}

%% Extra whitespace at the top.
\vspace*{2\bigskipamount}

%% Print the title.
{\makeatletter
\titlestyle\bfseries\LARGE\@title
\makeatother}

%% Print the optional subtitle.
{\makeatletter
\ifx\@subtitle\undefined\else
    \bigskip
    \titlefont\titleshape\Large\@subtitle
\fi
\makeatother}

\end{center}

\cleardoublepage
\thispagestyle{empty}

\begin{center}

%% The following lines repeat the previous page exactly.

\vspace*{2\bigskipamount}

%% Print the title.
{\makeatletter
\titlestyle\bfseries\LARGE\@title
\makeatother}

%% Print the optional subtitle.
{\makeatletter
\ifx\@subtitle\undefined\else
    \bigskip
    \titlefont\titleshape\Large\@subtitle
\fi
\makeatother}

%% Uncomment the following lines to insert a vertically centered picture into
%% the title page.
%\vfill
%\centering
\includegraphics{title}
\vfill

%% Apart from the names and dates, the following text is dictated by the
%% promotieregelement.

{\Large\titlefont\bfseries Proefschrift}

\bigskip
\bigskip

ter verkrijging van de graad van doctor

aan de Technische Universiteit Delft,

op gezag van de Rector Magnificus prof.~ir.~K.C.A.M.~Luyben,

voorzitter van het College voor Promoties,

in het openbaar te verdedigen op dinsdag 1 januari 2015 om 10:00 uur

\bigskip
\bigskip

door

\bigskip
\bigskip

%% Print the full name of the author.
\makeatletter
{\Large\titlefont\bfseries\@firstname\ {\titleshape\@lastname}}
\makeatother

\bigskip
\bigskip

Fachlehrer für Mathematik und Physik, \\
Eidgenössische Polytechnische Schule, Zürich, Zwitserland,

geboren te Ulm, Duitsland.

%% Extra whitespace at the bottom.
\vspace*{2\bigskipamount}

\end{center}

\clearpage
\thispagestyle{empty}

%% The following line is dictated by the promotieregelement.
\noindent Dit proefschrift is goedgekeurd door de

%% List the promotors (supervisors).
\medskip\noindent
\begin{tabular}{l}
    promotor: prof.\ dr.\ A.\ Kleiner \\
    copromotor: dr.\ A.A.\ Aaronson
\end{tabular}

\bigskip
\noindent Samenstelling promotiecommissie:

%% List the committee members, starting with the Rector Magnificus and the
%% promotor(s) and ending with the reserve members.
\medskip\noindent
\begin{tabular}{p{3cm}l}
    Rector Magnificus, & voorzitter \\
    Prof.\ dr.\ A.\ Kleiner, & Technische Universiteit Delft \\
    Dr.\ A.A.\ Aaronson, & Technische Universiteit Delft \\

    \medskip
    \mbox{\emph{Onafhankelijke leden:}} & \\

    Prof.\ dr.\ A.\ Jansen & Technische Universiteit Delft \\
    % Special case, only for very long names
    \mbox{Prof.\ dr.\ ir.\ A.B.C.D.\ van de Lange-Achternaam} & \\
      & Technische Universiteit Delft \\
    Prof.\.dr.\ N.\ Nescio & Politecnico di Milano, Itali\"e \\
    Prof.\ dr.\ ir.\ J.\ Doe, & Technische Universiteit Delft, reservelid \\

    \medskip
    \mbox{\emph{Overige leden:}} & \\
    Prof.\ dr.\ ir.\ J.\ de Wit, & Technische Universiteit Delft \\
    Dr.\ ir.\ Q.\ de Zwart, & Technische Universiteit Eindhoven \\
\end{tabular}

%% Include the following disclaimer for committee members who have contributed
%% to this dissertation. Its formulation is again dictated by the
%% promotieregelement.
\medskip
\noindent Prof.\ dr.\ ir.\ J.\ de Wit heeft in belangrijke mate aan de totstandkoming van het proefschrift bijgedragen.

%% Here you can include the logos of any institute that contributed financially
%% to this dissertation.
\vfill
\begin{center}
    \centering
\includegraphics[height=0.5in]{title/logos/tudelft}
    \hspace{2em}
    \centering
\includegraphics[height=0.5in]{title/logos/casimir} \\
    \centering
\includegraphics[height=0.5in]{title/logos/fom}
    \hspace{2em}
    \centering
\includegraphics[height=0.5in]{title/logos/nwo}
\end{center}
\vfill

\noindent
\begin{tabular}{@{}p{0.2\textwidth}@{}p{0.8\textwidth}}
    \textit{Keywords:} & \ldots \\[\medskipamount]
    \textit{Printed by:} & Johannes Gutenberg \\[\medskipamount]
    \textit{Front \& Back:} & Beautiful cover art that captures the entire content of this thesis in a single illustration.
\end{tabular}

\vspace{4\bigskipamount}

\noindent Copyright \textcopyright\ 2015 by A.~Einstein

%% Uncomment the following lines if this dissertation is part of the Casimir PhD
%% Series, or a similar research school.
%\medskip
%\noindent Casimir PhD Series, Delft-Leiden 2015-01

\medskip
\noindent ISBN 000-00-0000-000-0

\medskip
\noindent An electronic version of this dissertation is available at \\
\url{http://repository.tudelft.nl/}.

\end{titlepage}


